The Globalization Theorem for CD(K,N) on locally finite Spaces

We establish the local-to-global property of the synthetic curvature-dimension condition for essentially non-branching locally finite metric-measure spaces, extending the work [F. Cavalletti, E. Milman \textit{Invent. Math.} 226 (2021), no. 1, 1-137].

==> Conclusion.tex <==

As stated previously, $(X, d, \mathfrak{m})$ is an e.n.b. $\cd_{\loc}(K, N)$ geodesic m.m.s. with $\spt(\mathfrak{m})=X$. Fix $\mu_0, \mu_1 \in \mathcal{P}_2 (X, \mathfrak{m})$, and let $\varphi$ be an associated Kantorovich potential and $\nu$ be the unique optimal dynamical plan, concentrated on $G_{\varphi}$.

\subsection{$L^2$-Disintegration}\label{section:L2disint}
Given any Borel $G \subset G_{\varphi}$, in the style of disintegration, we
repeat two partitions in Section \ref{section:potentials} by taking
$\varphi_s \circ e_s$ and $\Phi_s^t$ be the quotient map $\mathfrak{Q}$
respectively:
\begin{enumerate}[label=(\Roman*)]
  \item $\mathfrak{Q}\colon (G, \nu) \rightarrow \im
  (\varphi_s \circ e_s) \subset \mathbb{R}$, with $G
  = \sqcup_{a_s} G_{a_s}$;
  \item $\mathfrak{Q}\colon (e_t (G), \mathfrak{m}) \rightarrow
  \im (\Phi_s^t) \subset \mathbb{R}$, with $e_t (G) =
  \sqcup_{a_s} e_t (G_{a_s})$.
\end{enumerate}
By Lemma $\ref{prop:continity}$, both quotient maps above are continuous.
If $G$ is compact, both $e_s (G)$ and $G_{a_s}$ are also compact,
so $\mathfrak{m} \llcorner e_t (G)$ is a finite measure. Applying Theorem
$\ref{thm:strongly cons}$, we have two disintegrations strongly
consistent with their quotient maps respectively:
\begin{enumerate}[label=(\Roman*)]
  \item Disintegration of $\nu \llcorner G$: $\varphi_s (e_s (G)) \ni a_s
  \mapsto \nu_{a_s} \in \mathcal{P} (\geo(X))$
  \begin{equation}
    \label{disint of nu} \nu = \int_{\varphi_s (e_s (G))} \nu_{a_s}
    \mathfrak{q}^{\nu}_s (\d a_s), \quad \nu_{a_s} (G_{a_s}) = 1,
  \end{equation}
  where $\mathfrak{q}^{\nu}_s = (\varphi_s \circ e_s)_{\#} \nu \llcorner G$ is
  the quotient measure on $\im (\varphi_s \circ e_s)$.
  
  \item\label{item:disint2} Disintegration of $\mathfrak{m} \llcorner e_t (G) : \varphi_s (e_s
  (G)) \ni a_s \mapsto \hat{\mathfrak{m}}^t_{a_s} \in \mathcal{P} (X)$
  \begin{equation}\label{disint of m|e_t(G)}
     \mathfrak{m} \llcorner e_t (G) =
    \int_{\varphi_s (e_s (G))} \hat{\mathfrak{m}}^t_{a_s} \mathfrak{q}^t_s (\d
    a_s), \quad \hat{\mathfrak{m}}^t_{a_s} (e_t (G_{a_s})) = 1, 
  \end{equation}
  where $\mathfrak{q}_s^t = (\Phi^t_s)_{\#} \mathfrak{m} \llcorner e_t (G)$ is
  the quotient measure on $\im (\Phi_s^t)$.
\end{enumerate}

\begin{proposition}[{\cite[Section 10.2]{cavalletti2021globalization}},
Absolute Continuity of Quotient Measures]\label{prop:queotient of nu is AC}
 Denote $G_{\varphi}^{ +} \coloneqq \{ \gamma
  \in G_{\varphi} : \ell (\gamma) > 0 \}$. When $G$ is a compact subset of
  $G_{\varphi}^+$,
  \begin{enumerate}
    \item For any $t, s, \tau \in (0, 1)$, quotient measures $\mathfrak{q}^t_s$ and
    $\mathfrak{q}^{\tau}_s$ are mutually absolutely continuous, both
    absolutely continuous to $\mathcal{L}^1$. We can rewrite \eqref{disint of m|e_t(G)} as
    \begin{equation} 
    \mathfrak{m} \llcorner e_t (G) = \int_{\varphi_s (e_s (G))}
       \mathfrak{m}^t_{a_s} \mathcal{L}^1 (\d a_s),\quad  \mathfrak{m}^t_{a_s} \coloneqq \frac{\d\mathfrak{q}^t_s}{\d\mathcal{L}^1} 
    \hat{\mathfrak{m}}^t_{a_s}. 
    \end{equation}
    \item For any $s \in (0, 1)$, quotient measures $\mathfrak{q}^{\nu}_s$
    and $\mathfrak{q}^s_s$ are mutually absolutely continuous, in particular
    $\mathfrak{q}^{\nu}_s\ll\mathcal{L}^1$. We can rewrite \eqref{disint of nu} as
    \begin{equation} 
    \nu = \int_{\varphi_s (e_s (G))} \nu_{a_s} q^{\nu}_s (a_s)
       \mathcal{L}^1(\d a_s),\quad q^{\nu}_s \coloneqq
    \frac{\d\mathfrak{q}^{\nu}_s}{\d\mathcal{L}^1}. 
       \end{equation}
  \end{enumerate}
\end{proposition}

As $(X, d, \mathfrak{m})$ is e.n.b., from \cref{lemma:injective}, $ \mu_t \llcorner e_t (G) = (e_t)_{\#}  (\nu \llcorner G)$ for all $t\in[0,1]$. Meanwhile, we have the trivial relation $\mu_t \llcorner e_t(G)=\rho_t\mathfrak{m}\llcorner e_t(G)$. So the two disintegrations in \cref{prop:queotient of nu is AC} imply two ways representing $\mu_t$ as follows
\begin{align}
  \mu_t \llcorner e_t (G) & =(e_t)_{\#}(\nu \llcorner G)=\int_{\varphi_s (e_s (G))} q^{\nu}_s (a_s)
  \cdot (e_t)_{\#} \nu_{a_s} \mathcal{L}^1 (\d a_s)\\
  & = \rho_t\mathfrak{m}\llcorner e_t(G)=\int_{\varphi_s (e_s (G))} \rho_t \cdot \mathfrak{m}^t_{a_s}\mathcal{L}^1 (\d a_s).
\end{align}
Both of them are strongly consistent with the partition $\sqcup_{a_s} e_t (G_{a_s})$ (by level sets of $\Phi^t_s$). Therefore by \cref{rmk:uniqueofdisinte}, for $\mathcal{L}^1$-a.e. $a_s \in \varphi_s (e_s (G))$
\begin{equation}
  \label{relation of condi. prob. 1} \rho_t \cdot \mathfrak{m}_{a_s}^t =
  q^{\nu}_s (a_s) \cdot (e_t)_{\#} \nu_{a_s} .
\end{equation}
For any Borel $H \subset G$, we integrate both sides of \eqref{relation of condi. prob. 1} over $e_t (H)$ to get
\begin{equation}
  \label{eq:combine of mu_t} \int_{e_t (H)} \rho_t (x)
  \cdot \mathfrak{m}^t_{a_s} (\d x) = q^{\nu}_s (a_s)  \int_{e_t (H)}
  (e_t)_{\#} \nu_{a_s} (\d x) = q^{\nu}_s (a_s) \nu_{a_s} (H),
\end{equation}
where the right-hand side does not depend on $t$.

\subsection{$L^1$-Disintegration}\label{section:L1dis}

\begin{definition}
  Given a continuous function $\phi : (X, d) \rightarrow \mathbb{R}$ with
  $\{ \phi = 0 \} \neq \emptyset$, define the \emph{signed distance function}
  (from zero-level set of $\phi$) as
  \begin{equation} 
  d_{\phi} : X \rightarrow \mathbb{R}, \qquad d_{\phi} (x) \coloneqq
     \mathrm{dist} (x, \{ \phi = 0 \}) \mathrm{sign} (\phi) . 
     \end{equation}
\end{definition}

Whenever $(X, d)$ is a length space, $d_{\phi}$ is $1$-Lipschitz. 

Let $(\varphi_t)_{t\in[0,1]}$ be the intermediate-time Kantorovich potentials of $\varphi$. For any $s \in
(0, 1)$ and $a_s \in \im (\varphi_s \circ e_s)$, denote $u \coloneqq d_{a_s} {\coloneqq d_{\phi}} $ as the signed
distance function from $\{ \varphi_s = a_s \}$. By
{\cite[Lemma 10.3]{cavalletti2021globalization}}, for every $\gamma \in G_{\varphi, a_s} \coloneqq \{ \gamma \in G_{\varphi} :
\varphi_s (\gamma_s) = a_s \}$ and $0 \leq r \leq t \leq 1$, $(\gamma_r, \gamma_t) \in R_u$. In particular, $e_{[0, 1]} (G_{\varphi, a_s}) \subset \mathcal{T}_u$.

Now we can further localize the ray decomposition in \cref{thm:transport set} to Kantorovich geodesics in $G_{\varphi, a_s}$. Take the new cross section $e_s (G_{\varphi, a_s})$ and define a Borel ray map
  $g^{a_s}$ as in \cref{def:ray map} but now fix the time variable to $[0, 1]$
  \begin{equation} 
  g^{a_s} : e_s (G_{\varphi, a_s}) \times [0, 1] \rightarrow X, \quad (\beta, t)
     \mapsto e_t (e_s^{-1} (\beta)) . 
     \end{equation}
A reformation on the disintegration of $\mathfrak{m} \llcorner e_{[0, 1]} (G_{\varphi, a_s})$ can be obtained by repeating \cite[Proposition
10.4]{cavalletti2021globalization}. Just notice that, regardless of whether $X$ has finite volume or not, conditional measures $(\m_q)_q$ are finite and compactly supported on some $\gamma\in G_{\varphi,a_s}$.

\begin{proposition}\label{thm:ray decomposition 2}
  For any compact subset $G \subset
  G_{\varphi}^+$ and $s \in (0, 1)$, $a_s \in \varphi_s (e_s (G))$, we have the following disintegration
  \begin{equation}\label{eq:ray decom of evolution}
    \mathfrak{m} \llcorner e_{[0, 1]} (G_{a_s}) = \int_{e_s (G_{a_s})} g^{a_s}
    (\beta, \cdot)_{\#} (h^{a_s}_{\beta} \cdot \mathcal{L}^1 \llcorner [0, 1])
    \mathfrak{q}^{a_s} (\d \beta), 
  \end{equation}
  where
  \begin{enumerate}
    \item $\mathfrak{q}^{a_s}$ is a finite Borel measure on $e_s (G_{a_s})$;
   
    \item\label{item:prop3.3(1)} the map $e_s (G_{a_s}) \times [0, 1] \ni (\beta, t) \mapsto
    h_{\beta}^{a_s} (t)$ is $\mathfrak{q}^{a_s} \otimes(\mathcal{L}^1
    \llcorner [0, 1])$-measurable;
    
    \item\label{itm:prop3.2(2)} $(h_{\beta}^{a_s})_{\beta}$ do not depend on choices of $G$;
    
    \item\label{item:prop3,3(3)} for $\mathfrak{q}^{a_s}$-a.e $\beta \in e_s (G_{a_s})$,
    $h_{\beta}^{a_s}$ is a $\cd (\ell^2_s (\beta) K, N)$ density satisfying $h_{\beta}^{a_s} (s) = 1$.
  \end{enumerate}
\end{proposition}

\begin{proof}[Brief discussion on the proof]
 Recall the disintegration over $\mathcal{T}_u$: 
 \[
 \mathfrak{m} \llcorner \mathcal{T}_u=\int_Q \m_q\mathfrak{q}(\d q).
 \]
The function $h_{\beta}^{a_s}$ is defined by the density of $\mathfrak{m}_q$ after
  conditioning it on $\gamma^{q} \coloneqq e_s^{- 1} (\beta)\subset R_u(q)$, where $\gamma^{q}$ is among curves in $G_{a_s}$ having non-empty intersection with $\mathcal{T}^b_u$. As a convex subspace of some $\cd(K,N)$ space, $(\gamma^q,d,\m_q)$ verifies $\cd(K,N)$. 
  Therefore, after rescaling the variable, the density $h^{a_s}_{\beta}$ on $[0,1]$ is a $\cd (\ell^2_s (\beta) K, N)$ density.
  
  Due to the compactness of $G$, the evolution $e_{[0,1]}(G)$ is bounded so by \eqref{ineq:locallyfinite}, $\m_q\llcorner \gamma^q$ has uniformly bounded volume. 
  After normalizing $\m_q$ (in which way we replace $\q$ by the weighted measure $\q^{a_s}\coloneqq \m_q(\gamma^q)\q$), we assume $h^{a_s}_{\beta}$ to be a probability density. 
  Notice for $\mathfrak{q}^{a_s}$-a.e $\beta$, the $\cd (\ell^2_s (\beta) K, N)$ density $h^{a_s}_{\beta}$ should be everywhere positive on $(0,1)$. 
  Further multiplying $\q^{a_s}$ by the positive $\q^{a_s}$-measurable function $\beta\mapsto h^{a_s}_{\beta}(s)$ allows us to fix $h^{a_s}_{\beta}(s)\equiv 1$. Besides, this procedure preserves the finiteness of $\q^{a_s}$ because $\cd(K,N)$ probability density on $(0,1)$ has uniform supremum which depends only on parameters $K,N$ (see the a-priori estimate \cite[Lemma A.8]{cavalletti2021globalization}).
\end{proof}

As $g^{a_s}$ disentangles $e_{[0, 1]} (G_{a_s})$ into the product of the
section $e_s (G_{a_s})$ and $[0, 1]$, we can invert the order of
integration in \eqref{eq:ray decom of evolution} by Fubini
(the measurability is ensured by \cref{thm:ray
decomposition 2}\eqref{item:prop3.3(1)}):
\begin{equation} 
\mathfrak{m} \llcorner e_{[0, 1]} (G_{a_s}) = \int_{[0, 1]}
   g^{a_s} (\cdot, t)_{\#} (h^{a_s}_{\cdot} (t) \cdot \mathfrak{q}
   \textsf{}^{a_s}) \mathcal{L}^1 (\d t) . 
   \end{equation}
By denoting $\mathfrak{m}^{a_s}_t \coloneqq g^{a_s} (\cdot, t)_{\#} 
(h^{a_s}_{\cdot} (t) \cdot \mathfrak{q}^{a_s})$, there follows a new
disintegration (measurability of $t \mapsto \mathfrak{m}^{a_s}_t$ comes from
the measurability of $g^{a_s}$ and $h$)
\begin{equation}
  \label{disinte formula 3} \mathfrak{m} \llcorner e_{[0, 1]}
  (G_{a_s}) = \int_{[0, 1]} \mathfrak{m}^{a_s}_t \mathcal{L}^1 (\d t),
\end{equation}
where $\mathfrak{m}^{a_s}_t$ is concentrated on $e_t (G_{a_s})$ for each $t
\in (0, 1)$ since $\mathfrak{q}^{a_s}$ is concentrated on $e_s (G_{a_s})$. In
particular, $\mathfrak{m}^{a_s}_s =\mathfrak{q}^{a_s}$ as $h_{\beta}^{a_s} (s) = 1$ for all $\beta$, and
\begin{equation}
  \mathfrak{m}^{a_s}_t = g^{a_s} (\cdot, t)_{\#}  (h^{a_s}_{\cdot} (t)
  \cdot \mathfrak{m}^{a_s}_s) . \label{eq:transitioncondim}
\end{equation}
Moreover, $e_t (G_{a_s})$ is mutually disjoint for different $t$ (see
\cite[Corollary 4.3]{cavalletti2021globalization}). So disintegration $\left(
\ref{disinte formula 3} \right)$ is strongly consistent with the partition
$e_{(0, 1)} (G_{a_s}) = \sqcup_t e_t (G_{a_s})$. In this way, by
restricting the disintegration \eqref{disinte formula 3} on
subinterval $(t - \varepsilon, t + \varepsilon)$, we have
\begin{equation} \label{eq:disinte formula 4}
  \mathfrak{m} \llcorner e_{(t - \varepsilon, t + \varepsilon)} (G_{a_s}) =
  \int_{t - \varepsilon}^{t + \varepsilon} \mathfrak{m}^{a_s}_{\tau}
  \mathcal{L}^1 \texttt{} (\d \tau) .
\end{equation}

Using relation \eqref{eq:transitioncondim} and a-priori estimate of $\cd(K,N)$ density, one can show that $(\m_{t}^{a_s})_t$ have uniformly bounded volume.
Further from disintegration \eqref{eq:disinte formula 4} and the uniform boundedness of $(\|\m^{a_s}_t\|)_t$, we can approximate $\m^{a_s}_t$ by restricting $\m$ to transporting bands converging to the slice $e_{t}(G_{a_s})$. 
These two assertions can be stated as the following lemma.

\begin{lemma}[{\cite[Proposition 10.7, Lemma 11.1]{cavalletti2021globalization}}]\label{lemma:approximate the slice by band}
     Let $G$ be a compact subset of $G^+_{\varphi}$.
     \begin{enumerate}
        \item\label{item:lemma3.5(1)}Given every $s \in (0, 1)$, for all $a_s \in \varphi_s (e_s (G))$, $t \in [0, 1] $
    \begin{equation} 
    \| \mathfrak{m}^{a_s}_t \| \leq C\mathfrak{m} (e_{[0, 1]} (G_{a_s})),
    \end{equation}
    where $C$ depends only on $K, N$ and $\hat{d} (G) \coloneqq \max\{ \ell (\gamma)^{- 1}, \ell (\gamma):\gamma \in G\}$.
    \item\label{item:lemma3.5(2)}The limit $\mathfrak{m}^{a_s}_t = \underset{\varepsilon \rightarrow 0}{\lim}
    \frac{1}{2 \varepsilon} \mathfrak{m} \llcorner e_{(t - \varepsilon, t +
    \varepsilon)} (G_{a_s})$ holds in the weak topology (dual of $C_b (X)$).
     \end{enumerate}
\end{lemma}

\subsection{Change-of-Variable Formula by Comparison of
Disintegrations}\label{section:cov}

Let $G$ be an arbitrary compact subset of $G_{\varphi}^+$ and $a_s \in
\im (\varphi_s \circ e_s)$ with fixed $s \in (0, 1)$.

In the preceding two subsections, we obtain disintegration $a_s \mapsto
\mathfrak{m}^t_{a_s}$ w.r.t. the ``inter level-set propagation'' $e_t
(G) = \sqcup_{a_s} e_t (G_{a_s})$ and disintegration $t \mapsto
\mathfrak{m}^{a_s}_t$ w.r.t. the ``intra level-set propagation'' $e_{[0, 1]}
(G_{a_s}) = \sqcup_t e_t (G_{a_s})$. Both $\mathfrak{m}^{a_s}_t$,
$\mathfrak{m}^t_{a_s}$ are concentrated on $e_t (G_{a_s})$, and it is shown by
Cavalletti-Milman in {\cite{cavalletti2021globalization}} that they are
equivalent up to derivative of $\Phi^t_s$.

\begin{theorem}[{\cite[Theorem 11.3]{cavalletti2021globalization}}]
  \label{thm:meascomp}For $\mathcal{L}^1$-a.e. t including $t = s$,
  \begin{enumerate}
    \item\label{item:thm3.5(1)} derivative $\partial_{\tau} \Phi^{\tau}_s |_{\tau = t}  (x)$ exists
    and it is positive for $\mathfrak{m}$-a.e. $x \in e_t (G^+_{\varphi})$ with
    \begin{equation} \partial_t \Phi^t_s (x) = \ell^2_t (x) + (t - s)  \frac{\partial_t
       \ell^2_t (x)}{2}, \quad \partial_{\tau} \Phi^{\tau}_s |_{\tau = s}
        (\gamma_s) = \ell_s^2 (\gamma_s) ; \end{equation}
    \item for $\mathcal{L}^1$-a.e. $a_s \in \varphi_s (e_s (G))$,
    $\mathfrak{m}^{a_s}_t = \partial_t \Phi^t_s \cdot \mathfrak{m}^t_{a_s}$
    and in particular $\mathfrak{m}^{a_s}_s = \ell_s^2 \cdot
    \mathfrak{m}^s_{a_s}$.
  \end{enumerate}
\end{theorem}

Part \eqref{item:thm3.5(1)} results from a purely metric-structure-based statement--\cref{lemma:derivativePhi}\eqref{item:lemma3.7(1)}. The second part is more complicated, but mainly based on \cref{lemma:approximate the slice by band} and \cref{lemma:derivativePhi}\eqref{item:lemma3.7(2)}.

\begin{lemma}[{\cite[Proposition
  4.4]{cavalletti2021globalization}}]\label{lemma:derivativePhi}
\indent\begin{enumerate}
   \item\label{item:lemma3.7(1)}  $\forall x \in X,$ $\partial_t \Phi^t_s (x)$ exists for
    $\mathcal{L}^1$-a.e. $t \in {G}_{\varphi} (x)$, including
    $t = s$ if $s \in {G}_{\varphi} (x)$, in which case
    $\partial_t |_{t = s}  \Phi^t_s (x) = \ell_s^2 (x)$.
    \item\label{item:lemma3.7(2)} There exist constants $C_t > 0$, locally bounded w.r.t. $t \in (0, 1)$ s.t.
    \begin{equation} 
    \partial_{\tau} \Phi^{\tau}_s |_{\tau = t}  (x) \leq C_t
     \sup_{\gamma \in G} \ell^2 (\gamma) \quad \text{a.e. $(x, t) \in D
     ({G}_{\varphi})$}.
     \end{equation}
\end{enumerate}
\end{lemma}

As all ingredients prepared, the change-of-variable formula follows as \cite[Theorem 11.4]{cavalletti2021globalization}.

\begin{theorem}[Change-of-Variable formula]
  \label{thm:cov}For any $s \in (0, 1)$, $\mathcal{L}^1$-a.e. $t \in (0, 1)$
  including $t = s$ and $\nu$-a.e. $\gamma \in G_{\varphi}^+$,
  $\partial_{\tau} |_{\tau = t} \Phi^{\tau}_s (\gamma_t)$ exists, positive and it holds
  \begin{equation}
    \frac{\rho_t (\gamma_t)}{\rho_s (\gamma_s)} = \frac{\partial_{\tau}
    |_{\tau = t} \Phi^{\tau}_s (\gamma_t)}{\ell^2 (\gamma)} \cdot
    \frac{1}{h^{\varphi_s (\gamma_s)}_{\gamma_s} (t)}, \label{eq:cov}
  \end{equation}
  where $h^{\varphi_s (\gamma_s)}_{\gamma_s}$ is a $\cd
  (\ell (\gamma)^2 K, N)$ density on $[0, 1]$ with $h^{\varphi_s(\gamma_s)}_{\gamma_s} (s) = 1$.
  
  In particular, Theorem \ref{thm:covIntro} is achieved by letting $h_s (t) =
  h^{\varphi_s (\gamma_s)}_{\gamma_s} (t)$ and $z (t) = \frac{\partial_{\tau}
  |_{\tau = t} \ell^2_{\tau} (\gamma_t)}{2 \ell^2 (\gamma)}$.
\end{theorem}

\begin{proof}
  ({\romannumeral 1}). Reduce to compact subsets.
  
  Given any compact $G \subset G^+_{\varphi}$ with $\nu (G) > 0$, $\tilde{\nu}
  \coloneqq \frac{1}{\nu (G)} \nu \llcorner G$ is an optimal dynamical plan. By
  \cref{thm:ray decomposition 2}\eqref{itm:prop3.2(2)}, function $h$ does not depend on $G$.
  If we can show for $\tilde{\nu}$-a.e. $\gamma \in G $, and
  $\mathcal{L}^1$-a.e. $t$ including $t = s$
  \begin{equation}
    \label{c.o.v.1} \tilde{\rho}_s (\gamma_s) \ell^{- 2} (\gamma) =
    \tilde{\rho}_t (\gamma_t) (\partial_{\tau} |_{\tau = t} \Phi^{\tau}_s
    (\gamma_t))^{- 1} h^{\varphi_s (\gamma_s)}_{\gamma_s} (t), \quad
    \tilde{\rho}_s = \frac{\d (e_t)_{\#} \tilde{\nu}}{\d\mathfrak{m}}
  \end{equation}
  then by the relation $\tilde{\rho}_s = (\nu (G))^{- 1} \rho_s \llcorner e_t
  (G)$, \eqref{eq:cov} is verified for $\nu$-a.e. $\gamma \in G$. 
  The inner regularity of $\nu$ ensures a sequence of compact subsets $G^n\subset G^+_{\varphi}$, $\nu (G^n) > 1 - 1 / n$ hence combining the justification of \eqref{c.o.v.1} for each $G^n$ completes the proof.
  
({\romannumeral 2}). Fix an arbitrary compact set $G$ of positive $\nu$-measure.
    Recalling \eqref{eq:combine of mu_t} in Section $\ref{section:L2disint}$ from comparing $L^2$-disintegrations of $\nu$ and $\mathfrak{m}
  \llcorner e_t (G)$, we have for any $s, t \in
  (0, 1)$ and any Borel $H\subset G$,
  \begin{equation}\label{eq:4.7}
   \int_{e_t (H)} \rho_t (x) \cdot \mathfrak{m}^t_{a_s}
    (\d x) = q^{\nu}_s (a_s) \nu_{a_s} (H),\quad \mathcal{L}^1\text{-a.e. }a_s \in \varphi_s (e_s (G)).
  \end{equation}
 If we take $T \coloneqq
  \left\{ t \in [0, 1] : \text{Theorem $\ref{thm:meascomp}$ holds at $t$}
  \right\}$, then $s \in T$ and $\mathcal{L}^1 (T) = 1$. At $t \in T$, replacing
  $\mathfrak{m}^t_{a_s}$ by $(\partial_t \Phi^t_s)^{- 1}
  \mathfrak{m}^{a_s}_t$, and using the transferring formula \eqref{eq:transitioncondim}, we get
  \begin{eqnarray}
    q^{\nu}_s (a_s) \nu_{a_s} (H) & = & \int_{e_t (H)} \rho_t (x) (\partial_t
    \Phi^t_s)^{- 1} \mathfrak{m}^{a_s}_t (\d x) \nonumber\\
    & = & \int_{g^{a_s} (\cdot, t) (e_s (H))} \rho_t (x)  (\partial_t
    \Phi^t_s)^{- 1} g^{a_s} (\cdot, t)_{\#}  (h^{a_s}_{\cdot} (t) \cdot
    \mathfrak{m}^{a_s}_s)  (\d x) \nonumber\\
    & = & \int_{e_s (H)} (\rho_t (\partial_t \Phi^t_s)^{- 1}) \circ g^{a_s}
    (\beta, t) h^{a_s}_{\beta} (t) \mathfrak{m}^{a_s}_s (\d \beta) . 
    \label{eq:separate s,t prove cov}
  \end{eqnarray}
 Let $f_t (\beta) \coloneqq (\rho_t (\partial_t \Phi^t_s)^{- 1}) \circ g^{a_s} (\beta, t) h^{a_s}_{\beta} (t)$. As the measure $\mathfrak{m}^{a_s}_s$
  is frozen, by arbitrariness of $H$, $f_t (\beta) = f_{\tilde{t}}(\beta)$ for all $t, \tilde{t} \in T$, $\mathfrak{m}^{a_s}_s$-a.e. $\beta
  \in e_s (G)$ and $\mathcal{L}^1$-$a_s \in \varphi_s (e_s (G))$. In
  particular, since $h^{a_s}_{\beta} (s) = 1$ and $\partial_t |_{t = s}  \Phi^t_s (\gamma_s) = \ell_s^2(\gamma_s)$ take $\tilde{t} = s$,
  \begin{equation}\label{eq:compare
    density step 3 bad measure}
    (\rho_t (\partial_t \Phi^t_s)^{- 1}) \circ g^{a_s} (\beta, t)
    h^{a_s}_{\beta} (t) = (\ell^2_s (\beta))^{- 1} \rho_s (\beta), \quad
    \text{$\mathfrak{m}^{a_s}_s$-a.e. $\beta \in e_s (G)$}. 
  \end{equation}
  
  Again by Theorem $\ref{thm:meascomp}$, measures $\mathfrak{m}^{a_s}_s$ and
  $\mathfrak{m}_{a_s}^s$ are mutually absolutely continuous, so $\left(
  \ref{eq:compare density step 3 bad measure} \right)$ holds for
  $\mathfrak{m}_{a_s}^s$-a.e. $\beta \in e_s (G)$ as well. The validity of
  \eqref{eq:compare density step 3 bad measure} for almost each
  $a_s$ indicates that, after recovering measure $\mathfrak{m} \llcorner e_s
  (G)$ by $\int_{\varphi_s (e_s (G))} \mathfrak{m}^s_{a_s} \mathcal{L}^1 (\d
  a_s)$, \eqref{eq:compare density step 3 bad measure} holds for $\mathfrak{m}$-a.e. (so $\mu_s$-a.e) $\beta\in e_s(G)$.
  
  Hence, replacing $\beta$ by $\gamma_s$ in \eqref{eq:compare density
  step 3 bad measure} for $\nu$-a.e. $\gamma \in G$ and $\mathcal{L}^1$-a.e. $t \in (0, 1)$, we have
  \begin{equation} \rho_t (\gamma_t) (\partial_t \Phi^t_s)^{- 1} (\gamma_t)
     h_{\gamma_s}^{\varphi_s (\gamma_s)} (t) = (\ell_s^2 (\gamma_s))^{- 1}
     \rho_s (\gamma_s) . 
     \end{equation}
     
  ({\romannumeral 3}). As $\mu_t \ll \mathfrak{m}$, from Theorem
  $\ref{thm:meascomp}$, the derivative $\partial_{\tau} |_{\tau = t}
  \Phi^{\tau}_s (x)$ exists for $\mu_t$-a.e. $x \in e_t (G)$ which is just the
  differentiability of $\tau \mapsto \Phi^{\tau}_s (\gamma_t)$ at $\tau = t$
  along $\nu$-a.e. $\gamma$. And
  \begin{equation} \frac{\partial_{\tau} |_{\tau = t} \Phi^{\tau}_s (\gamma_t)}{\ell^2
     (\gamma)} = \left( \ell^2_t (\gamma_t) + (t - s)  \frac{\partial_t
     \ell^2_t (\gamma_t)}{2} \right) \frac{1}{\ell^2 (\gamma)} = 1 + (t - s) z
     (t) . \end{equation}
  Finally, \cite[Theorem 5.2, Subsection 12.1]{cavalletti2021globalization} show there is a Lipschitz version of
  $z$ satisfying $z' \geq z^2$.
\end{proof}

\subsection{Comments on the Globalization Theorem}\label{section:comments}
\subsubsection*{From change-of-variable formula to pointwise inequality of $\cd(K,N)$} A formal proof of \eqref{eq:CDKNintro} can be immediately produced from \cref{thm:cov} if we assume $\left(
\ref{eq:covIntro} \right)$ to hold strictly everywhere for $s, t \in (0, 1)$
and all functions are $C^2$. Indeed, fix some $a \in (0, 1)$ and define
\begin{equation} Y (r) = \exp \left( \int_a^r \partial_t |_{t = s} \log h_s (t) \d s
   \right), \quad L (r) = \exp \left( - \int_a^r z (s) \d s \right) . \end{equation}
One can check from \eqref{eq:covIntro}, $\frac{\rho_a
(\gamma_a)}{\rho_r (\gamma_r)} = Y (r) L (r)$. Moreover, $L$ is concave from $z'
\geq z^2$ and $Y$ is a $\cd (\ell (\gamma)^2 K, N)$ density by the
following calculation:
\begin{eqnarray}
  &  & \frac{((\log Y)')^2}{N - 1} (r) + (\log Y)'' (r) \nonumber\\
  & = & \frac{(\partial_t |_{t = r} \log h_r (t))^2}{N - 1} + \partial_t^2
  |_{t = r} \log h_r (t) + \partial_s \partial_t |_{t = s = r} \log h_s (t)
  \nonumber\\
  & \overset{\left( \ref{eq:covIntro} \right)}{=} & \frac{(\partial_t |_{t =
  r} \log h_r (t))^2}{N - 1} + \partial_t^2 |_{t = r} \log h_r (t) +
  \partial_s \partial_t |_{t = s = r} \log (1 + (t - s) z (t)) \nonumber\\
  & = & \frac{(\partial_t |_{t = r} \log h_r (t))^2}{N - 1} + \partial_t^2
  |_{t = r} \log h_r (t) - z' (r) + z^2 (r) \overset{\eqref{eq:AppendCD}}{\leq} - \ell (\gamma)^2 K,
  \label{ineq:Yintro}
\end{eqnarray}
where the inequality based on the fact that $h_s$ is a $\cd (\ell (\gamma)^2 K,
N)$ density. Then \eqref{eq:CDKNintro} follows from this ``$Y-L$" disentanglement of $t
\mapsto \rho_t (\gamma_t)$ once applying H\"{o}lder's inequality.

A rigorous proof without the extra regularity assumption is given by \cite[Section 12]{cavalletti2021globalization}. The idea is to mollify
$h_s (t)$ by taking logarithmic convolution on both variable $s, t$ 
\begin{equation}
    \log h^{\varepsilon_1,\varepsilon_2}_s(t)\coloneqq \iint \log h_y(x)\psi_{\varepsilon_1}(t-x)\psi_{\varepsilon_2}(s-y)\d x\d y
    \end{equation}
and show that the inequality \eqref{ineq:Yintro} holds for the new $Y^{\varepsilon_1,\varepsilon_2}$ up to some inessential error. 
As $\cd(K,N)$ for density functions can be preserved under pointwise convergence, the proof will be completed if one can show the pointwise limit of $h^{\varepsilon_1,\varepsilon_2}_s(t)$ to $h^s(t)$ when $\varepsilon_1,\varepsilon_2\rightarrow 0$. 

\subsubsection*{On null-geodesics} Deriving the distorted inequality \eqref{eq:CDKNintro} for null-geodesics (curve in $G_{\varphi} \setminus G^+_{\varphi}$, or simply curve of a single point) is less involved, which can be found in \cite[Theorem 11.4, Step 0]{cavalletti2021globalization}.
Roughly speaking, we can always redefine the density on null-geodesics with only
negligible influence on each $\mu_t$ by letting
\begin{equation} \rho_s (\gamma_s) = \rho_t (\gamma_t), \quad \forall t, s \in [0, 1],
   \gamma \in G_{\varphi} \setminus G^+_{\varphi} . \end{equation}

\subsubsection*{$\cd^1$-conditions} In \cite{cavalletti2021globalization}, the authors introduced the notion of $\cd^1$ condition.
Basically, it requires a disintegration of $\m\llcorner \mathcal{T}_u$ for any 1-Lipschitz function $u$ so that almost each conditional measure is a probability measure and \eqref{item:unique}-\eqref{itm:1.3.4} in \cref{thm:ray decomposition1} are satisfied. 
The globalization theorem is proved by completing the chain
\begin{equation}\label{eq:chain}
    \cd_{\loc}(K,N)\Rightarrow \cd^1(K,N)\Rightarrow \cd(K,N).
\end{equation}

We can extend the definition of $\cd^1(K,N)$ to locally-finite spaces by replacing the assumption $\m_q(X_q)=1$ with \cref{thm:ray decomposition1}\eqref{itm:locallyfinite}. Then the uniform boundedness over any bounded set is sufficient for all localization and conditioning arguments involved for concluding $\cd^1(K,N)\Rightarrow \cd(K,N)$.

To expand this assertion, notice first of all  a repetition of \cite[Section 8.2]{cavalletti2021globalization} ensures
\[
\mcp^1(K,N)\Rightarrow \mcp(K,N).
\]
Thus the whole story can start with the presence of local compactness, properness and the continuity of dynamics (\cref{thm:densityconti}).
Further, in \cref{section:L2disint}-\cref{section:cov}, we were actually following arguments in \cite{cavalletti2021globalization} on showing $\cd(K,N)$ by $\cd^1(K,N)$ (actually $\cd^1_{\mathrm{Lip}}(K,N)$). Whenever \eqref{ineq:locallyfinite} is enforced, conditional measures in \cref{thm:ray decomposition 2} restricted on Kantorovich geodesics have finite volumes (and if we do not insist on the normalization $h^{a_s}_{\beta}(s)=1$, $\m_q\llcorner \gamma^q$ can be a probability measure), producing the $L^1$-disintegration and all subsequent statements we need.

Together with \cref{thm:ray decomposition1}, we can complete the chain \eqref{eq:chain} on locally-finite spaces.



